Stimulating Diffusion Model for Image Denoising via Adaptive Embedding and Ensembling

Image denoising is a fundamental problem in computational photography, where achieving high perception with low distortion is highly demanding. Current methods either struggle with perceptual quality or suffer from significant distortion. Recently, the emerging diffusion model has achieved state-of-the-art performance in various tasks and demonstrates great potential for image denoising. However, stimulating diffusion models for image denoising is not straightforward and requires solving several critical problems. For one thing, the input inconsistency hinders the connection between diffusion models and image denoising. For another, the content inconsistency between the generated image and the desired denoised image introduces distortion. To tackle these problems, we present a novel strategy called the Diffusion Model for Image Denoising (DMID) by understanding and rethinking the diffusion model from a denoising perspective. Our DMID strategy includes an adaptive embedding method that embeds the noisy image into a pre-trained unconditional diffusion model and an adaptive ensembling method that reduces distortion in the denoised image. Our DMID strategy achieves state-of-the-art performance on both distortion-based and perception-based metrics, for both Gaussian and real-world image denoising.The code is available at https://github.com/Li-Tong-621/DMID.

==> Figures/psnr-sure.tex <==
\begin{figure}[t!]
    \begin{center}
        \subfigure[]{
        %\label{FPN_k}
            \includegraphics[width=0.46\columnwidth]{Images/psnr-sure/1.pdf}
        }
        \subfigure[]{
        %\label{FPN_b}
            \includegraphics[width=0.46\columnwidth]{Images/psnr-sure/2.pdf}
        }\vspace{-2pt}
        \subfigure[]{
        %\label{t-dependent}
            \includegraphics[width=0.46\columnwidth]{Images/psnr-sure/3.pdf}
            }
        \subfigure[]{
        %\label{t-independent}
            \includegraphics[width=0.46\columnwidth]{Images/psnr-sure/4.pdf}
        }\vspace{-2pt}
    \end{center}
    \vspace{-6pt}
    \caption{
    Every 500 iterations, we employ SURE to determine whether to stop the noise transformation. A higher value of “-SURE” indicates better image quality. (a)-(d) illustrate the changes in PSNR and -SURE during the noise transformation process. In usual cases, the variations in -SURE align with those of PSNR.
    }
    \label{fig:psnr-sure}
\end{figure}

==> Figures/realworld.tex <==
\begin{figure*}[!t]
\footnotesize
\renewcommand{\arraystretch}{1.2}
\begin{center}
\setlength{\tabcolsep}{1.5pt}
\scalebox{0.97}{
\begin{tabular}[b]{c c c c c c c c}
% \hspace{-4mm}


\multirow{4}{*}{\includegraphics[trim={0 0 0 0},clip,width=.245\textwidth,valign=t]{Images/realworld/cc1/noisy_draw.png}}&
% \includegraphics[trim={224 224 224 224},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/noisy.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/DaNet.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/MIRNet.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/MPRNet.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/DeamNet.png} &  
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/NAFNet.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/Uformer.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/restormer_g.png} 
\\
& 32.38 / 0.1532
& 31.94 / 0.1885
& 31.94 / 0.1946
& 32.20 / 0.1917
& 31.66 / {\color{blue}0.1457}
& 32.21 / 0.1808
& 31.53 / 0.1929
\\

&DaNet$_+$%~\cite{ECCV2020_984}
&MIRNet%~\cite{MIR}
&MPRNet%~\cite{zamir2021multi}
&DeamNet%~\cite{ren2021adaptivedeamnet}
&NAFNet%~\cite{chen2022simple} 
&Uformer%~\cite{wang2022uformer}
% &\small{Restormer$_g$~\cite{zamir2022restormer}}
&Restormer$_g$
\\
&
%left bottom right top
%\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/restormer_r.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/AP-BSN.png} & 
 \includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/LG-BPN.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/R2R.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/ZS-N2N.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/DMID-d.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/DMID-p.png} & 
\includegraphics[trim={192 175 256 273},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/clean.png} 
\\
%29.63 / 0.2868
32.02 / 0.1752
&32.02 / 0.2128
& 32.08 / 0.2169
&29.65 / 0.2871
&29.77 / 0.2789
% &{\color{red}35.55 /}{ \color{blue}0.1297}
% &{\color{blue}34.37 /}{ \color{red} 0.0779}
% &{\color{red}35.37 /}{ \color{blue}0.1512}
% &{\color{blue}35.28 /}{ \color{red} 0.1511}
&{\color{red}35.11 /}{ \color{black}0.1624}
&{\color{blue}34.84 /}{ \color{red} 0.1235}
&PSNR / LPIPS

\\
% &\small{Restormer$_r$~\cite{zamir2022restormer}}

Noisy
%&Restormer$_r$
&AP-BSN%~\cite{lee2022apbsn}
&LG-BPN%~\cite{wang2023lgbpn}
&R2R%~\cite{Recorrupted2Recorrupted}
&ZS-N2N%~\cite{ZSNoise2Noise} 
% & \textbf{DMID-d (Ours)}
% & \textbf{DMID-p (Ours)} 
& \textbf{DMID-d}
& \textbf{DMID-p} 
&Clean
\\
% %left bottom right top
% %%%%第二张图片 CC2
% Noisy 
% %&Noisy
% &DaNet$_+$%~\cite{ECCV2020_984}
% &MIRNet%~\cite{MIR}
% &MPRNet%~\cite{zamir2021multi}
% &DeamNet%~\cite{ren2021adaptivedeamnet}
% &NAFNet%~\cite{chen2022simple} 
% &Uformer%~\cite{wang2022uformer}
% % &\small{Restormer$_g$~\cite{zamir2022restormer}}
% &Restormer$_g$
% \\

% \multirow{4}{*}{\includegraphics[trim={0 0 0 0},clip,width=.245\textwidth,valign=t]{Images/realworld/cc2/noisy.png}}&
% % \includegraphics[trim={224 224 224 224},clip,width=.1\textwidth,valign=t]{Images/realworld/cc1/noisy.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/DaNet.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/MIRNet.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/MPRNet.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/DeamNet.png} &  
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/NAFNet.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/Uformer.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/restormer_g.png} 
% \\
% & 32.72 / 0.1175
% & 32.29 / 0.1477
% & 32.03 / 0.1628
% & 32.43 / 0.1509
% & 32.08 / 0.1287
% & 32.41 / 0.1366
% & 32.33 / 0.1211
% \\
% % &\small{Restormer$_r$~\cite{zamir2022restormer}}
% &Restormer$_r$
% &AP-BSN%~\cite{lee2022apbsn}
% % &LG-BPN~\cite{wang2023lgbpn}
% &R2R%~\cite{Recorrupted2Recorrupted}
% &ZS-N2N%~\cite{ZSNoise2Noise} 
% % & \textbf{DMID-d (Ours)}
% % & \textbf{DMID-p (Ours)} 
% & \textbf{DMID-d}
% & \textbf{DMID-p} 
% &Clean
% \\
% &
% %left bottom right top
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/restormer_r.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/AP-BSN.png} & 
% % \includegraphics[trim={224 224 224 224},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/LG-BPN.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/R2R.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/ZS-N2N.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/DMID-d.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/DMID-p.png} & 
% \includegraphics[trim={300 320 40 20},clip,width=.1\textwidth,valign=t]{Images/realworld/cc2/clean.png} 
% \\
% 29.87 / 0.2960
% &32.15 / 0.1499
% &31.97 / 0.2222
% %& 31.83 / 0.1995
% &29.91 / 0.2952
% &29.93 / 0.2920
% &{\color{red}34.43 / 0.0937}
% &{\color{blue}33.85 / 0.0928}
% &PSNR / LPIPS

% \\
%left bottom right top
%%%%第3张图片 polyu1


% \multirow{4}{*}{\includegraphics[trim={0 0 0 0},clip,width=.245\textwidth,valign=t]{Images/realworld/polyu1/noisy_draw.png}}&
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/DaNet.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/MIRNet.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/MPRNet.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/DeamNet.png} &  
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/NAFNet.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/Uformer.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/restormer_g.png} 
% \\
% &  35.47 / 0.1219
% & 35.46 / 0.1440
% & 35.77 / 0.1361
% & 32.57 / 0.1314
% & 34.13 / 0.1299
% & 35.68 / 0.1347
% & 35.08 / 0.1492


% \\
% &DaNet$_+$%~\cite{ECCV2020_984}
% &MIRNet%~\cite{MIR}
% &MPRNet%~\cite{zamir2021multi}
% &DeamNet%~\cite{ren2021adaptivedeamnet}
% &NAFNet%~\cite{chen2022simple} 
% &Uformer%~\cite{wang2022uformer}
% % &\small{Restormer$_g$~\cite{zamir2022restormer}}
% &Restormer$_g$
% \\

% &
% %left bottom right top
% %\includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/restormer_r.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/AP-BSN.png} & 
%  \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/LG-BPN.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/R2R.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/ZS-N2N.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/DMID-d.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/DMID-p.png} & 
% \includegraphics[trim={80 0 270 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu1/clean.png} 
% \\
% 34.54 / 0.1638

% &34.14 / 0.1410
% & 33.70 / 0.1660
% &34.50 / 0.1289
% &34.57 / 0.1636
% % &{\color{red}37.18 /}{ \color{blue} 0.0412}
% % &{\color{blue}36.95 /}{ \color{red} 0.0398}
% % &{\color{red}37.19 /}{ \color{blue} 0.0677}
% % &{\color{blue}37.06 /}{ \color{red} 0.0657}
% &{\color{red}34.63 /}{ \color{blue} 0.1566}
% &{\color{blue}34.45 /}{ \color{red} 0.1560}
% &PSNR / LPIPS

% \\
% Noisy
% %&Restormer$_r$
% &AP-BSN%~\cite{lee2022apbsn}
% &LG-BPN%~\cite{wang2023lgbpn}
% &R2R%~\cite{Recorrupted2Recorrupted}
% &ZS-N2N%~\cite{ZSNoise2Noise} 
% % & \textbf{DMID-d (Ours)}
% % & \textbf{DMID-p (Ours)} 
% & \textbf{DMID-d}
% & \textbf{DMID-p} 
% &Clean
% \\
%%%%%polyu3


\multirow{4}{*}{\includegraphics[trim={0 0 0 0},clip,width=.245\textwidth,valign=t]{Images/realworld/polyu3/noisy.png}}&
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/DaNet.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/MIRNet.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/MPRNet.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/DeamNet.png} &  
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/NAFNet.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/Uformer.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/restormer_g.png} 
\\
& 37.04 / 0.1462
& 36.84 / 0.1666
& 36.99 / 0.1690
& 32.95 / 0.1677
& 36.28 / 0.1599
& 36.93 / 0.1564
& 36.19 / 0.2079


\\
&DaNet$_+$%~\cite{ECCV2020_984}
&MIRNet%~\cite{MIR}
&MPRNet%~\cite{zamir2021multi}
&DeamNet%~\cite{ren2021adaptivedeamnet}
&NAFNet%~\cite{chen2022simple} 
&Uformer%~\cite{wang2022uformer}
% &\small{Restormer$_g$~\cite{zamir2022restormer}}
&Restormer$_g$
\\

&
%left bottom right top
%\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/restormer_r.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/AP-BSN.png} & 
 \includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/LG-BPN.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/R2R.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/ZS-N2N.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/DMID-d.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/DMID-p.png} & 
\includegraphics[trim={0 0 350 350},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu3/clean.png} 
\\
35.36 / 0.2316

&36.56 / 0.1074
&36.07 / 0.1212
&35.78 / 0.1824
&35.37 / 0.2315
% &{\color{red}37.18 /}{ \color{blue} 0.0412}
% &{\color{blue}36.95 /}{ \color{red} 0.0398}
% &{\color{red}37.19 /}{ \color{blue} 0.0677}
% &{\color{blue}37.06 /}{ \color{red} 0.0657}
&{\color{red}39.54 /}{ \color{blue} 0.0658}
&{\color{blue}39.37 /}{ \color{red} 0.0607}
&PSNR / LPIPS

\\
Noisy
%&Restormer$_r$
&AP-BSN%~\cite{lee2022apbsn}
&LG-BPN%~\cite{wang2023lgbpn}
&R2R%~\cite{Recorrupted2Recorrupted}
&ZS-N2N%~\cite{ZSNoise2Noise} 
% & \textbf{DMID-d (Ours)}
% & \textbf{DMID-p (Ours)} 
& \textbf{DMID-d}
& \textbf{DMID-p} 
&Clean
\\


%left bottom right top
%%%%第4张图片 polyu2

\multirow{4}{*}{\includegraphics[trim={0 0 0 0},clip,width=.245\textwidth,valign=t]{Images/realworld/polyu2/noisy_draw.png}}&
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/DaNet.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/MIRNet.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/MPRNet.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/DeamNet.png} &  
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/NAFNet.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/Uformer.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/restormer_g.png} 
\\
& 37.07 / 0.1075
& 37.41 / 0.1155
& 37.03 / 0.1204
& 37.51 / 0.1156
& 37.15 / 0.1337
& 37.72 / 0.1057
& 36.84 / 0.1289

\\
&DaNet$_+$%~\cite{ECCV2020_984}
&MIRNet%~\cite{MIR}
&MPRNet%~\cite{zamir2021multi}
&DeamNet%~\cite{ren2021adaptivedeamnet}
&NAFNet%~\cite{chen2022simple} 
&Uformer%~\cite{wang2022uformer}
% &\small{Restormer$_g$~\cite{zamir2022restormer}}
&Restormer$_g$
\\

&
%left bottom right top
%\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/restormer_r.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/AP-BSN.png} & 
 \includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/LG-BPN.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/R2R.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/ZS-N2N.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/DMID-d.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/DMID-p.png} & 
\includegraphics[trim={387 0 0 387},clip,width=.1\textwidth,valign=t]{Images/realworld/polyu2/clean.png} 
\\
34.86 / 0.2063
% 36.92 / 0.1267
&37.57 / 0.1113
& 37.90 / 0.1322
&35.27 / 0.1546
&34.86 / 0.2063
% &{\color{red}38.79 /}{ \color{blue} 0.0987}
% &{\color{blue}38.31 /}{ \color{red}0.0896}
% &{\color{red}39.33 /}{ \color{blue} 0.0993}
% &{\color{blue}39.17 /}{ \color{red}0.0939}
&{\color{red}39.22 /}{ \color{blue}0.0998}
&{\color{blue}39.05 /}{ \color{red}0.0954}

&PSNR / LPIPS

\\
Noisy
%&Restormer$_r$
&AP-BSN%~\cite{lee2022apbsn}
&LG-BPN%~\cite{wang2023lgbpn}
&R2R%~\cite{Recorrupted2Recorrupted}
&ZS-N2N%~\cite{ZSNoise2Noise} 
% & \textbf{DMID-d (Ours)}
% & \textbf{DMID-p (Ours)} 
& \textbf{DMID-d}
& \textbf{DMID-p} 
&Clean
\\

\end{tabular}}
\end{center}
%\vspace*{-2mm}

\caption{Visual results on real-world image denoising. Our method achieves better denoising results and pictures restored by our method are more detailed and realistic. 
}
\label{fig:realworld}
%\vspace{-0.5em}
\end{figure*}

==> Tables/2_realworld_old.tex <==
%%%PSNR↑ / LPIPS↓ / FID↓
%\begin{table*}[t!]
%%\small
%\caption{Real-world image denoising. Our method achieves SOTA performance across all metrics (PSNR↑ / LPIPS↓ / FID↓) when compared to both supervised and unsupervised methods. The best and second-best methods are in {\color{red}red} and {\color{blue}blue}.} 
%\label{table:1-real}
%\renewcommand{\arraystretch}{1.2}
%\setlength{\tabcolsep}{1pt}
%\scalebox{0.99}{
%    \begin{tabular}{c c c| c c c| c c c |c c c }
%    \toprule
%    {\makebox[0.04\textwidth][c]{}}
%    &{\makebox[0.15\textwidth][c|]{}} 
%    &{\makebox[0.12\textwidth][c]{}}
%    & \multicolumn{3}{c|}{CC~\cite{2016A}}
%    & \multicolumn{3}{c|}{PolyU~\cite{xu2018real}} 
%    & \multicolumn{3}{c}{FMDD~\cite{zhang2018poisson}}
%    
%    \\ 
%    \cline{4-12} 
%    \multirow{-2}{*}{Type of supervision}
%    &\multirow{-2}{*}{Training data}
%    &\multirow{-2}{*}{Method}  
%    & {\makebox[0.06\textwidth][c]{PSNR}} 
%    & {\makebox[0.06\textwidth][c]{LPIPS}}
%    & {\makebox[0.06\textwidth][c]{FID}}
%    & {\makebox[0.06\textwidth][c]{PSNR}} 
%    & {\makebox[0.06\textwidth][c]{LPIPS}} 
%    & {\makebox[0.06\textwidth][c]{FID}}
%    & {\makebox[0.06\textwidth][c]{PSNR}} 
%    & {\makebox[0.06\textwidth][c]{LPIPS}} 
%    & {\makebox[0.06\textwidth][c]{FID}}
%
%    \\ 
%    \midrule
%
%    {}
%    &{}
%    &DaNet$_+$~\cite{ECCV2020_984}
%    & 35.91 & 0.073 & 49.9
%    & 37.25 & 0.088 & 40.7
%    & 31.59 & 0.238 & 174 
%    \\
%    {}
%    &{}
%    &MIRNet~\cite{MIR}
%    & 36.04 & 0.088 & 54.3
%    & 37.45 & 0.101 & 35.5
%    & 31.83 & 0.227 & 180
%    
%    \\
%    {}
%    &{}
%    &MPRNet~\cite{zamir2021multi}
%    & 36.20 & 0.094 & 59.5
%    & 37.43 & 0.109 & 35.6
%    & 31.21 & 0.292 & 240
%    \\
%    {}
%    &{}
%    &DeamNet~\cite{ren2021adaptivedeamnet}
%    & 35.64 & 0.089 & 57.2
%    & 32.46 & 0.130 & 53.4
%    & 32.28 & 0.261 & 225
%    {}
%    \\
%    &{}
%    &NAFNet~\cite{chen2022simple} 
%    & 34.39 & 0.073 & 56.6
%    & 36.09 & 0.107 & 44.6
%    & 26.27 & 0.340 & 254
%    {}
%    \\
%    &{}
%    &Uformer~\cite{wang2022uformer}
%    & 36.31 & 0.085 & 53.5
%    & 37.31 & 0.096 & 33.9
%    & 31.81 & \color{blue}{0.207} &  \color{blue}{165}
% 
%    \\
%    {}
%    &{}
%    &Restormer$_g$~\cite{zamir2022restormer}
%    & 35.28 & 0.121 & 69.9
%    & 37.09 & 0.121 & 44.9
%    & 31.50 & 0.250 & 173
%    
%    \\
%    \multirow{-8}{*}{Supervised}
%    &\multirow{-8}{*}{Real noisy-clean pairs}
%    &Restormer$_r$~\cite{zamir2022restormer}
%    &  36.27 & 0.077 & 50.7
%    &  37.51 & 0.102 & \color{blue}{33.4}
%    &  31.81 & 0.211 & 180
%    
%    \\
%    \midrule
%    {}
%    &{}
%    &N2V~\cite{noise2void}
%    &32.27 & - & -
%    &33.83 & - & -
%    &- & - & -
%    
%
%    \\
%    {}
%    &{}
%    &N2S~\cite{noise2self}
%    &33.38 & - & -
%    &35.04 & - & -
%    &- & - & -
%
%    \\
%    {}
%    &{}
%    &AP-BSN~\cite{lee2022apbsn}
%    & 34.86 & 0.134 & 86.4
%    & 36.45 & 0.099 & 46.5
%    & 32.40 & 0.335 & 257
%    \\
%    {}
%    &\multirow{-4}{*}{Real noisy dataset}
%    &LG-BPN~\cite{wang2023lgbpn}
%    & 34.58 & 0.135 & 92.8
%    & 36.59 & 0.102 & 52.4
%    & 33.12 & 0.283 & 206
%
%    \\
%    \cline{2-12} 
%    % {}
%    % &{}
%    % &S2S~\cite{self2self}
%    % &35.27 & 0.143 & 67.8
%    % &- & - & -
%    % &- & - & -
%    % \\
%    {}
%    &{}
%    &R2R~\cite{Recorrupted2Recorrupted}
%    &33.43 & 0.227 & 84.4
%    &36.23 & 0.151 & 42.6
%    &27.17 & 0.448 & 211
%    
%    \\
%    {}
%    &{}
%    &ZS-N2N~\cite{ZSNoise2Noise}
%    &33.51 & 0.224 & 82.4
%    &35.99 & 0.197 & 46.4
%    &31.65 & 0.222 & 177
%    \\
%    
%    {}
%    &{}
%    &\textbf{DMID-d (Ours)}
%    &  \color{red}{38.19} & \color{blue}{0.055} & \color{blue}{49.2}
%    &  \color{red}{38.85} & \color{red}{0.050} & \color{black}{34.2}
%    &  \color{red}{34.02} & \color{black}{0.238} & 200
%
%    \\
%    \multirow{-8}{*}{Unsupervised}
%    &\multirow{-4}{*}{Single noisy observation}
%    &\textbf{DMID-p (Ours)}
%    & \color{blue}{37.74} & \color{red}{0.052} & \color{red}{48.5}
%    & \color{blue}{38.53} & \color{blue}{0.051} & \color{red}{32.3}
%    & \color{blue}{33.57} & \color{red}{0.171} & \color{red}{160}
%
%    \\
%    \bottomrule %[0.1em]
%    
%    \end{tabular}%
%
%}
%
%%\vspace{-1em}
%\end{table*}





\begin{table*}[t!]
	%\small
	\caption{Real-world image denoising. Our method achieves SOTA performance across all metrics (PSNR↑ / SSIM↑ / LPIPS↓) when compared to both supervised and unsupervised methods. The best and second-best methods are in {\color{red}red} and {\color{blue}blue}.} 
	\label{table:1-real}
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{1pt}
	\scalebox{0.99}{
		\begin{tabular}{c |c |c| c c c| c c c |c c c }
			\toprule
			{\makebox[0.04\textwidth][c]{}}
			&{\makebox[0.15\textwidth][c|]{}} 
			&{\makebox[0.12\textwidth][c]{}}
			& \multicolumn{3}{c|}{CC~\cite{2016A}}
			& \multicolumn{3}{c|}{PolyU~\cite{xu2018real}} 
			& \multicolumn{3}{c}{FMDD~\cite{zhang2018poisson}}
			
			\\ 
			\cline{4-12} 
			\multirow{-2}{*}{Type of supervision}
			&\multirow{-2}{*}{Training data}
			&\multirow{-2}{*}{Method}  
			& {\makebox[0.06\textwidth][c]{PSNR}} 
			& {\makebox[0.06\textwidth][c]{SSIM}}
			& {\makebox[0.06\textwidth][c]{LPIPS}}
			& {\makebox[0.06\textwidth][c]{PSNR}} 
			& {\makebox[0.06\textwidth][c]{SSIM}} 
			& {\makebox[0.06\textwidth][c]{LPIPS}}
			& {\makebox[0.06\textwidth][c]{PSNR}} 
			& {\makebox[0.06\textwidth][c]{SSIM}} 
			& {\makebox[0.06\textwidth][c]{LPIPS}}
			
			\\ 
			\midrule
			
			{}
			&{}
			&DaNet$_+$~\cite{ECCV2020_984}
			&35.91 &0.9816 &\color{blue}{0.073}
			&37.23 &0.9796 &0.088
			&31.59 &0.7962 &0.238
			\\
			{}
			&{}
			&MIRNet~\cite{MIR}
			&36.04 &0.9797 &0.088
			&37.45 &0.9783 &0.101
			&31.83 &0.8106 &0.227
			
			\\
			{}
			&{}
			&MPRNet~\cite{zamir2021multi}
			&36.20 &0.9769 &0.094
			&37.43 &0.9759 &0.109
			&31.21 &0.7915 &0.292
			\\
			{}
			&{}
			&DeamNet~\cite{ren2021adaptivedeamnet}
			&35.64 &0.9652 &0.089
			&32.46 &0.8615 &0.130
			&32.28 &0.8116 &0.261
			{}
			\\
			&{}
			&NAFNet~\cite{chen2022simple} 
			&34.39 &0.9784 &\color{blue}{0.073}
			&36.04 &0.9607 &0.107
			&26.27 &0.6519 &0.340
			{}
			\\
			&{}
			&Uformer~\cite{wang2022uformer}
			&36.31 &0.9795 &0.085
			&37.31 &0.9782 &0.096
			&31.81 &0.8118 &\color{red}{0.207}
			
			\\
			{}
			&{}
			&Restormer$_g$~\cite{zamir2022restormer}
			&35.28 &0.9745 &0.121
			&37.09 &0.9731 &0.121
			&31.50 &0.7654 &0.250
			
			\\
			\multirow{-8}{*}{Supervised}
			&\multirow{-8}{*}{Real noisy-clean pairs}
			&Restormer$_r$~\cite{zamir2022restormer}
			&36.27 &0.9810 &0.077
			&37.51 &0.9776 &0.102
			&31.81 &0.8046 & \color{blue}{0.211}
			
			\\
			\midrule
			{}
			&{}
			&N2V~\cite{noise2void}
			&32.27 & 0.8620 & -
			&33.83 & 0.8730 & -
			&- & - & -
			
			
			\\
			{}
			&{}
			&N2S~\cite{noise2self}
			&33.38 & 0.8460 & -
			&35.04 & 0.9020 & -
			&- & - & -
			
			\\
			{}
			&{}
			&AP-BSN~\cite{lee2022apbsn}
			&34.86 &0.9744 &0.131
			&36.45 &0.9750 &0.099
			&32.40 &0.8461 &0.335
			\\
			{}
			&\multirow{-4}{*}{Real noisy dataset}
			&LG-BPN~\cite{wang2023lgbpn}
			&34.58 &0.9755 &0.135
			&36.59 &0.9763 &0.102
			&33.12 &0.8668 &0.283
			\\
			\cline{2-12} 
			 {}
			 &{}
			 &S2S~\cite{self2self}
%			 &35.27 & 0.143 & 67.8
			 &37.52 & 0.9510 & -
			 &38.37 & 0.9620 & -
			 &- & - & -
			 \\
			{}
			&{}
			&R2R~\cite{Recorrupted2Recorrupted}
			&33.43 &0.9564 &0.227
			&36.23 &0.9655 &0.151
			&27.17 &0.5250 &0.448
						
			\\
			{}
			&{}
			&ZS-N2N~\cite{ZSNoise2Noise}

			&33.51 &0.9571 &0.224
			&35.99 &0.9587 &0.197
			&31.65 &0.7674 &0.222
			\\
			
			&
			&  \textbf{DMID-d (Ours)}
			& \color{red}{38.36} & \color{red}{0.9892}  & \color{black}{0.075}
			&  \color{red}{38.93} & \color{red}{0.9861} & \color{blue}{0.063}
			&  \color{red}{33.92} & \color{red}{0.8982} & 0.237
			
			\\
			\multirow{-9}{*}{Unsupervised}
			&\multirow{-5}{*}{Single noisy observation}
			&\textbf{DMID-p (Ours)}
			&\color{blue}{38.12} & \color{blue}{0.9887}  & \color{red}{0.072}
			&\color{blue}{38.79} & \color{blue}{0.9853}  & \color{red}{0.059}
			&\color{blue}{33.65} & \color{blue}{0.8774}  & \color{black}{0.224}
			
			\\
			\bottomrule %[0.1em]
			
		\end{tabular}%
		
	}
\end{table*}
	%\vspace{-1em}\end{table*}


==> Tables/4_diffusion_real.tex <==
% \begin{table}[t!]
% \small
% \caption{Compared with other diffusion-based methods on real-world denoising.}
% \label{table:4-diffusion-real}
% \setlength{\tabcolsep}{1pt}
% \scalebox{0.99}{
%     \begin{tabular}{c c c c }
%     \toprule
%     {\makebox[0.05\textwidth][c]{}} &
%     {\makebox[0.13\textwidth][c]{DDRM~\cite{kawar2022denoising}}} & 
%     {\makebox[0.13\textwidth][c]{DDNM~\cite{wang2022zero}}} & 
%     {\makebox[0.13\textwidth][c]{\textbf{DMID-d (Ours)}}} 

%     \\ 
%     \cline{2-4} 
%     \multirow{-2}{*}{Dataset}
%     & PSNR / LPIPS / FID
%     & PSNR / LPIPS / FID
%     & PSNR / LPIPS / FID
%     \\ 
%     \midrule

%     CC

%     &  36.02 / {\color{blue}0.073 / 49.6}
%     &  {\color{blue}37.43} / 0.076 / 54.2	 
%     %&  \color{red}{37.74} / \color{red}{0.052} / \color{red}{48.5}
%     &  \color{red}{38.19} / \color{red}{0.055} / \color{red}{49.2}
    
    
%     \\
    
%     PolyU
%     & 36.86 / 0.088 / {\color{blue}51.2}
%     & {\color{blue}38.84 / 0.061} / 56.5
%     %&  \color{red}{38.53} / \color{red}{0.051} / \color{red}{32.3}
%     &  \color{red}{38.85} / \color{red}{0.050} / \color{red}{34.2}
    
%     \\
    
%     FMDD
%     & 32.81 / {\color{blue}0.316 / 269}
%     & {\color{blue}33.13} / 0.332 / 277
%     %&  \color{red}{33.57} / \color{red}{0.171} / 160 
%     &  \color{red}{34.02} / \color{red}{0.238} / 200 
%     \\
    
%     \bottomrule[0.1em]
    
%     \end{tabular}%

% }

% \vspace{-1em}
% \end{table}





%\begin{table}[t!]
%%\small
%\caption{Compared with other diffusion-based methods on real-world denoising.}
%\label{table:4-diffusion-real}
%\setlength{\tabcolsep}{1.5pt}
%\renewcommand{\arraystretch}{1.2}
%\scalebox{0.99}{
%    \begin{tabular}{c c c c }
%    \toprule
%    {\makebox[0.05\textwidth][c]{}} &
%    {\makebox[0.13\textwidth][c]{DDRM~\cite{kawar2022denoising}}} & 
%    {\makebox[0.13\textwidth][c]{DDNM~\cite{wang2022zero}}} & 
%    {\makebox[0.13\textwidth][c]{\textbf{DMID-d (Ours)}}} 
%
%    \\ 
%    \cline{2-4} 
%    \multirow{-2}{*}{Dataset}
%    & PSNR / LPIPS / FID
%    & PSNR / LPIPS / FID
%    & PSNR / LPIPS / FID
%    \\ 
%    \midrule
%
%    CC
%
%    &  {\color{blue}33.52 / 0.221 / 82.9}
%    &  {\color{blue}33.52} / 0.222 / 83.3	 
%    % &  \color{red}{37.06} / \color{red}{0.065} / \color{red}{44.8}
%
%    &  \color{red}{38.19} / \color{red}{0.055} / \color{red}{49.2}
%    
%    
%    \\
%    
%    PolyU
%    & 36.00 / {\color{blue}0.196 / 46.0}
%    & {\color{blue}36.01 / 0.196} / 46.2
%    &  \color{red}{38.85} / \color{red}{0.050} / \color{red}{34.2}
%    
%    \\
%    
%    FMDD
%    & {\color{blue}27.23 / 0.450 /} 205
%    & {\color{black}27.22} / 0.452 / {\color{blue}204}
%    &  \color{red}{34.02} / \color{red}{0.238} / 200 
%    \\
%    
%    \bottomrule%[0.1em]
%    
%    \end{tabular}%
%
%}
%
%%\vspace{-1em}
%\end{table}



\begin{table}[t!]
	%\small
	\caption{Compared with other diffusion-based methods on real-world denoising.}
	\label{table:4-diffusion-real}
	\setlength{\tabcolsep}{1.5pt}
	\renewcommand{\arraystretch}{1.2}
	\scalebox{0.95}{
		\begin{tabular}{c c c c }
			\toprule
			{\makebox[0.05\textwidth][c]{}} &
			{\makebox[0.13\textwidth][c]{CC~\cite{2016A}}} & 
			{\makebox[0.13\textwidth][c]{PolyU~\cite{xu2018real}}} & 
			{\makebox[0.13\textwidth][c]{FMDD~\cite{zhang2018poisson}} }
			
			\\ 
			\cline{2-4} 
			\multirow{-2}{*}{Method}
			& PSNR / SSIM / LPIPS
			& PSNR / SSIM / LPIPS
			& PSNR / SSIM / LPIPS
			\\ 
			\midrule
			
			DDRM
			
			&33.52 / 0.9575 / 0.221
			&36.00 / 0.9590 / 0.196
			&27.23 / 0.5451 / 0.450
			
			\\
			DDRM$^*$
			
			&{\color{black}36.03 / 0.9788 / 0.081}
			&{\color{black}38.07 / 0.9828 /} {\color{red}0.057}
			&{\color{black}29.61 / 0.7156 / 0.291}
			
			\\
			
			DDNM
			& 33.52 / 0.9575 / 0.222
			& 36.01 / 0.9590 / 0.196
			& 27.22 / 0.5442 / 0.450
			
			\\
			DDNM$^*$
			& 35.27 / 0.9723 / 0.126
			& 36.94 / 0.9700 / 0.133
			& 29.18 / 0.6790 / 0.328
			
			\\
			
			\textbf{DMID-d}
			&  {\color{red}38.36 / 0.9892 /} {\color{blue}0.075}
			&  {\color{red}38.93 / 0.9861 /} {\color{black}0.063}
			&  {\color{red}33.92 / 0.8982 /} {\color{blue} 0.237 }
			
			\\
			
			\textbf{DMID-p}
			&\color{blue}{38.12} / \color{blue}{0.9887}  / \color{red}{0.072}
			&\color{blue}{38.79} / \color{blue}{0.9853}  / \color{blue}{0.059}
			&\color{blue}{33.65} / \color{blue}{0.8774}  / \color{red}{0.224}
			\\
			
			\bottomrule%[0.1em]
			
		\end{tabular}%
		
	}
	
	%\vspace{-1em}
\end{table}


==> Tables/6_noise.tex <==

\begin{table}[t!]
	%\small
	\caption{Effectiveness of noise transformation.}
	\label{table:6-noise}
	\setlength{\tabcolsep}{1.5pt}
	\renewcommand{\arraystretch}{1.2}
	\scalebox{0.99}{
		\begin{tabular}{c c c c }
			\toprule
			{\makebox[0.08\textwidth][c]{ Covert to}} &
            {\makebox[0.08\textwidth][c]{Noise}} &
			{\makebox[0.13\textwidth][c]{CC}} & 
			{\makebox[0.13\textwidth][c]{PolyU}} 
			
			\\ 
			\cline{3-4} 
			% \multirow{-2}{*}{Intermediate}
			% &\multirow{-2}{*}{Transformation}
                {$x_N$}
                & Transformation
			& PSNR / SSIM / LPIPS
			& PSNR / SSIM / LPIPS
			\\ 
			\midrule
			
			\Checkmark
                & \XSolidBrush
			
			&\color{blue}{35.97 / 0.0000} / 0.000
			&\color{blue}{37.89 / 0.0000} / 0.000
			
			\\
			\Checkmark
			& \Checkmark
			&\color{red}{37.44 / 0.9859} / 0.082
			&\color{red}{38.79 / 0.9853} / 0.059
			
			\\
			\bottomrule%[0.1em]
		\end{tabular}%
	}
\end{table}


==> Tables/9_time.tex <==
\begin{table}[ht]
\begin{center}
\caption{The comparison of denoising runtime for single image ($512\times512\times1$) from FMDD dataset. 
}
\label{table:9_time}
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{2pt}
\scalebox{1}{
    \begin{tabular}{c| c c c c c}
    \toprule
    {}
    % &{Restormer}&{LG-BPN}
    % &{DDRM}&{DDNM}&{DM+Ours}&{DMID-d (Ours)}&{DMID-p (Ours)}
    &{DDRM}&{DDNM}&{DM+Ours}&{DMID-d}&{DMID-p}
    \\
     \midrule
    {Runtime/s}
   % &0.42
   % &92.08
   &11.42
   &57.38
   &8.00
   &581.42
   &1.16
   \\ 
    \bottomrule
    \end{tabular}%
}
\end{center}
\end{table}



\begin{table}[ht]
\begin{center}
\caption{The comparison of denoising runtime for single image ($512\times512\times1$) from FMDD dataset. 
}
\label{table:9_time}
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{2pt}
\scalebox{0.95}{
    \begin{tabular}{c| c c c c c}
    \toprule
    {}
    % &{Restormer}&{LG-BPN}
    % &{DDRM}&{DDNM}&{DM+Ours}&{DMID-d (Ours)}&{DMID-p (Ours)}
    &{DDRM}&{DDNM}&{DM+Ours}&{DMID-d (Ours)}&{DMID-p (Ours)}
    \\
     \midrule
    {Runtime/s}
   % &0.42
   % &92.08
   &11.42
   &57.38
   &8.00
   &581.42
   &1.16
   \\ 
    \bottomrule
    \end{tabular}%
}
\end{center}
\end{table}


\begin{table}[ht]
\begin{center}
\caption{The comparison of denoising runtime for single image ($512\times512\times1$) from FMDD dataset. 
}
\label{table:9_time}
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{2pt}
\scalebox{0.9}{
    \begin{tabular}{c| c c c c c c c}
    \toprule
    {}
    &{Restormer}&{LG-BPN}
    &{DDRM}&{DDNM}&{DM+Ours}&{DMID-d}&{DMID-p}
    \\
     \midrule
    {Runtime/s}
   &0.42
   &92.08
   &11.42
   &57.38
   &8.00
   &581.42
   &1.16
   \\ 
    \bottomrule
    \end{tabular}%
}
\end{center}
\end{table}

